Universal Semi-Supervised Semantic Segmentation

In recent years, the need for semantic segmentation has arisen across several different applications and environments. However, the expense and redundancy of annotation often limits the quantity of labels available for training in any domain, while deployment is easier if a single model works well across domains. In this paper, we pose the novel problem of universal semi-supervised semantic segmentation and propose a solution framework, to meet the dual needs of lower annotation and deployment costs. In contrast to counterpoints such as fine tuning, joint training or unsupervised domain adaptation, universal semi-supervised segmentation ensures that across all domains: (i) a single model is deployed, (ii) unlabeled data is used, (iii) performance is improved, (iv) only a few labels are needed and (v) label spaces may differ. To address this, we minimize supervised as well as within and cross-domain unsupervised losses, introducing a novel feature alignment objective based on pixel-aware entropy regularization for the latter. We demonstrate quantitative advantages over other approaches on several combinations of segmentation datasets across different geographies (Germany, England, India) and environments (outdoors, indoors), as well as qualitative insights on the aligned representations.

==> scripts/path_abs.tex <==
\begin{abstract}

    Modern deep learning based algorithms combined with large scale datasets have pushed the boundaries of performance on semantic segmentation tasks to a great extent. However current training methods are limited to giving good accuracies within a particular domain, and traditional fine tuning/adaptation based methods necessitate training separate models for each of the domains. In this paper, we propose a semi-supervised universal segmentation framework to train a single joint model on multiple domains, each of which has few labeled examples but large number of unlabeled examples. We use a pixel level entropy regularization based feature alignment objective to include the large amounts of unlabeled data in the training process. Training such a joint model on diverse domains, for example on different cities in case of autonomous driving, provides us with considerable deployment efficiency. Results on several challenging segmentation datasets further prove the effectiveness of the proposed framework. 
    
\end{abstract}



==> scripts/path_intro.tex <==
\section{Introduction}
\label{sec:intro}

In computer vision, semantic segmentation is the task of pixel level classification of an image into a predefined set of categories, which finds applications in natural scene understanding~\cite{GARCIAGARCIA201841} and medical imaging~\cite{ronneberger2015u}.
Most segmentation architectures~\cite{long2015fully, badrinarayanan2015segnet, chen2018deeplab} pre-train deep networks on a classification task on datasets like ImageNet~\cite{deng2009imagenet, russakovsky2015imagenet}, and then fine tune on large amounts of finely annotated labeled examples~\cite{cordts2016cityscapes, anue}. They show encouraging results when trained and tested within the same domain, but the performance hurts even in the presence of a minor domain shift. For example, a segmentation model trained on a driving dataset collected and curated in a specific geographical location does not show satisfactory performance when deployed in a new city due to minor differences which might arise in lighting conditions, weather conditions or traffic volume that are usually not discernible to the human eye. 
% Similarly, segmentation models trained on indoor datasets fails to correctly segment images from an outdoor environment, although the same objects are present in both cases. 
Since it is a highly prohibitive and redundant exercise to collect data for different locations and tasks separately due to the enormous costs of human effort and time involved in annotation, there is a growing interest towards learning shareable representations applicable across domains. 

\begin{figure}[!t]
\centering
  \includegraphics[width=0.9\linewidth]{Figures/IntroPic.pdf}
\vspace{-2em}
    \caption{Proposed universal segmentation model can be jointly trained across datasets with different label spaces, making use of the large amounts of unlabeled data available. Traditional domain adaptation and transfer learning based approaches can degrade accuracies in the source domain when finetuned/adapted to the target domain.}
\label{fig:intro_pic}
\vspace{-2em}
\end{figure}

%% Taxonomy paper for multitask motivation

Previous works on domain adaptation from a labeled source domain to an unlabeled target domain address this problem of domain shift in semantic segmentation~\cite{hoffman2016fcns, tsai2018learning, chen2017no, murez2018image,carlucci2017auto}. However, most of these works assume that the target label set matches with the source label set which does not accurately depict the general use case with semantic segmentation datasets. For instance, there might be many region specific label categories in case of driving datasets and fine tuning separate models for each domain comes with a huge deployment overhead. This is also true in case of driving datasets and indoor segmentation datasets, which have completely non-overlapping categories between them even though they share many useful relationships.
%although they share the same lower level representations. 
%So there is a need to perform universal transfer of representations in a label efficient manner across low resource domains.

To this end, we develop a universal semantic segmentation framework by aggregating knowledge from several different domains during training, each of which has very few labeled examples but several unlabeled examples. First proposed in ~\cite{liang2018dynamic}, universal segmentation is inspired by the success in joint multitask learning on diverse domains, datasets and tasks~\cite{kokkinos2017ubernet, mccann2018natural, kaiser2017one}. Compared to training separate models, multitask training is shown to improve performance on each of the individual tasks, due to better sharing of useful relationships between them~\cite{zamir2018taskonomy}. In this work, we build a universal semantic segmentation framework by training a single joint model on multiple domains, and make use of the large number of unlabeled examples to align the pixel level deep feature representations from multiple domains with the help of an entropy regularization based objective function. We calculate the similarity score vector between the features and the label embeddings computed from class prototypes~\cite{snell2017prototypical}, and minimize the entropy of this discrete distribution to positively align similar examples between the labeled and the unlabeled images.

%% We can collect datasets from "representative" cities and use the jointly trained model in any new city.
% In our case, it helps to align the visual features of multiple domains in a common subspace, by enforcing each feature to be close to one label.

In summary, we make the following contributions:
\begin{itemize}
    \item We propose a universal segmentation framework to train a single joint model on multiple domains with disparate label spaces to improve performance on each of the domains.
    
    \item We introduce a pixel level entropy regularization objective to train semantic segmentation architectures using datasets with very few labeled examples and large number of unlabeled examples.
    
    \item We demonstrate the effectiveness of the proposed framework over a combination of wide variety of indoor~\cite{song2015sun} and outdoor~\cite{cordts2016cityscapes, anue, brostow2009semantic} semantic segmentation datasets. We use dilated residual networks in our experiments, but the framework is agnostic to the particular deep segmentation network used and can be used with any of the existing encoder decoder architectures.
    
    % \item We show that the universal segmentation model helps to learn transferable features not only across similar domains, but also across widely different domains, like indoor objects and autonomous driving datasets, which further showcases the effectiveness of having shared lower level representations across tasks and datasets. 
    
\end{itemize}

The rest of the paper is organized as follows. \secref{sec:related} summarizes existing literature in areas related to our work while \secref{sec:problem_description} explains the problem setup and the proposed solution. \secref{sec:results} provides experimental validation to the proposed idea on multiple datasets and \secref{sec:conclusion} finally concludes the paper. 




==> scripts/qualt.tex <==
\begin{figure*}
\vspace{-0.5em}
\centering
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/ANUE_image_159.png}
                \vspace{-2em}
                % \caption{\label{fig:anue_image}}        
                
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/ANUE_bad_pred_159.png}
                \vspace{-2em}
                % \caption{\label{fig:anue_bad}}
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/ANUE_good_pred_159.png}
                \vspace{-2em}
                % \caption{\label{fig:anue_good}}
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/ANUE_label_159.png}
                \vspace{-2em}
                % \caption{\label{fig:anue_label}}         
                
        \end{subfigure}\hfill
        %
        ~
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CS_image_491.png}
                % \vspace{-2.5em}
                % \caption{\label{fig:cs_image}}
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CS_bad_pred_491.png}
                % \vspace{-2.5em}
                % \caption{\label{fig:cs_bad}}
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CS_good_pred_491.png}
                % \vspace{-2.5em}
                % \caption{\label{fig:cs_good}}
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CS_label_491.png}
                % \vspace{-2.5em}
                % \caption{\label{fig:cs_label}}
        \end{subfigure}\hfill
        % \caption{}
        ~
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CVD_image_115.png}
                \vspace{-1.5em}
                \caption{Original Image\label{fig:cvd_image}}
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CVD_bad_pred_115.png}
                \vspace{-1.5em}
                \caption{Without Entropy Module\label{fig:cvd_bad}}
        \end{subfigure}\hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CVD_good_pred_115.png}
                \vspace{-1.5em}
                \caption{With Entropy Module\label{fig:cvd_good}}
        \end{subfigure} \hfill
        %
        \begin{subfigure}[b]{0.248\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/Qualt/CVD_label_115.png}
                \vspace{-1.5em}
                \caption{Ground Truth Segmentation\label{fig:cvd_label}}
        \end{subfigure}\hfill
        %
        \captionsetup{width=0.95\textwidth}
        \caption{Qualitative examples from each dataset training with and without the proposed entropy regularization module. The first row shows example from IDD dataset, second row from Cityscapes and the third from the CamVid dataset.}
        \label{fig:qualitative}
        % \bigskip
        % \vspace{-1em}
\end{figure*}

